Active Learning with Selective Time-Step Acquisition for PDEs

Accurately solving partial differential equations (PDEs) is critical to understanding complex scientific and engineering phenomena, yet traditional numerical solvers are computationally expensive. Surrogate models offer a more efficient alternative, but their development is hindered by the cost of generating sufficient training data from numerical solvers. In this paper, we present a novel framework for active learning in PDE surrogate modeling that reduces this cost. Unlike the existing AL methods for PDEs that always acquire entire PDE trajectories, our approach, STAP (**S**elective **T**ime-Step **A**cquisition for **P**DEs), strategically generates only the most important time steps with the numerical solver, while employing the surrogate model to approximate the remaining steps. This reduces the cost incurred by each trajectory and thus allows the active learning algorithm to try out a more diverse set of trajectories given the same budget. To accommodate this novel framework, we develop an acquisition function that estimates the utility of a set of time steps by approximating its resulting variance reduction. We demonstrate the effectiveness of our method on several benchmark PDEs.

==> figure/acq_explanation.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[width=0.4\textwidth]{figure/variance_reduction.png}
    \caption{Illustration of variance reduction}
    \label{fig:acq_explanation}
\end{figure}


==> figure/base_burgers/base_burgers.tex <==
\begin{figure*}[htbp]
    \centering
    % First subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_burgers/random.png}
        \caption{Random}
        \label{fig:random}
    \end{subfigure}
    % Second subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_burgers/qbc.png}
        \caption{QbC}
        \label{fig:qbc}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_burgers/lcmd.png}
        \caption{LCMD}
        \label{fig:lcmd}
    \end{subfigure}

    \caption{Log RMSE of base methods with and without \gls{stap} on Burgers, measured across 10 rounds of acquisition.}
    \label{fig:base_burgers}
\end{figure*}


==> figure/base_ns/base_ns.tex <==
\begin{figure*}[htbp]
    \centering
    % First subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_ns/random.png}
        \caption{Random}
        \label{fig:random}
    \end{subfigure}
    % Second subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_ns/qbc.png}
        \caption{QbC}
        \label{fig:qbc}
    \end{subfigure}
    % Third subfigure
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/base_ns/lcmd.png}
        \caption{LCMD}
        \label{fig:lcmd}
    \end{subfigure}

    \caption{RMSE of base methods with and without \gls{stap} on NS, measured across 10 rounds of acquisition.}
    \label{fig:base_ns}
\end{figure*}


==> figure/concept.tex <==

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figure/concept.png}
%     \caption{Conceptual illustration of our framework.}
% \label{fig:explanation}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/explanation_v2.png}
    \caption{Conceptual illustration of our method and previous work. {Each dot represents a PDE state, and a path connecting two dots represents a time step of a simulation. Black solid lines are obtained with a numerical solver and red dotted lines with a surrogate model.}}
    \label{fig:concept}
\end{figure}


==> figure/gt_pred/gt_pred.tex <==

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/gt_pred/burgers.png}
        \caption{Burgers}
    \end{subfigure}
    % \hfill
    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/gt_pred/kdv.png}
        \caption{KdV}
    \end{subfigure}

    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/gt_pred/ks.png}
        \caption{KS}
    \end{subfigure}
    % \hfill
    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/gt_pred/ins.png}
        \caption{INS}
    \end{subfigure}
      % \vspace{0.5cm} % Adjust space between subfigures

    \caption{Ground truth versus predicted trajectories}
    \label{fig:gt_pred}
\end{figure}


==> figure/kdv_energy.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[width=0.4\textwidth]{figure/kdv_energy.png}
    \caption{Energy of KdV states in ground truth trajectory and prediction by a surrogate model.}
    \label{fig:kdv_energy}
\end{figure}


==> figure/ks_rmse.tex <==
\begin{figure}[t]
    \centering
        \includegraphics[width=0.8\textwidth]{figure/ks_rmse.png}
    \caption{An instance of model prediction in KS equation with RMSE of 0.958.}
    \label{fig:ks_rmse}
\end{figure}


==> figure/main_nrmse/main_nrmse.tex <==

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/main_nrmse/burgers.png}
        \caption{Burgers}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figure/main_nrmse/kdv.png}
        \caption{KdV}
    \end{subfigure}
    
    \vspace{0.1cm} % Adjust space between subfigures
    
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figure/main_nrmse/ks.png}
        \caption{KS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=0.98\textwidth]{figure/main_nrmse/ns.png}
        \caption{NS}
    \end{subfigure}

    \caption{Log NRMSE of AL strategies, measured across 10 rounds of acquisition. Each round incurs constant cost of data acquisition, namely the budget $B$.}
    \label{fig:main_nrmse}
\end{figure}


==> figure/main_old/main.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/burgers.png} % Scaled image
        \caption{Burgers}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/kdv.png} % Scaled image
        \caption{KdV}
    \end{subfigure}
    \hfill
    % \vspace{0.1cm} % Adjust space between subfigures
    \begin{subfigure}{0.24\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/ks.png} % Scaled image
        \caption{KS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/ns.png} % Scaled image
        \caption{NS}
    \end{subfigure}

    \caption{Log RMSE of AL strategies, measured across 10 rounds of acquisition. Each round incurs constant cost of data acquisition, namely the budget $B$.}
    \label{fig:main}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/burgers.png} % Scaled image
%         \caption{Burgers}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/kdv.png} % Scaled image
%         \caption{KdV}
%     \end{subfigure}
%     % \vspace{0.1cm} % Adjust space between subfigures
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/ks.png} % Scaled image
%         \caption{KS}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/ns.png} % Scaled image
%         \caption{NS}
%     \end{subfigure}

%     \caption{Log RMSE of AL strategies, measured across 10 rounds of acquisition. Each round incurs constant cost of data acquisition, namely the budget $B$.}
%     \label{fig:main}
% \end{figure*}

==> figure/main_old2/main.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.19\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/burgers.png} % Scaled image
        \caption{Burgers}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/kdv.png} % Scaled image
        \caption{KdV}
    \end{subfigure}
    \hfill
    % \vspace{0.1cm} % Adjust space between subfigures
    \begin{subfigure}{0.19\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/ks.png} % Scaled image
        \caption{KS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/ns.png} % Scaled image
        \caption{INS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth} % Reduced width
        \centering
        \includegraphics[width=\textwidth]{figure/main/cns.png} % Scaled image
        \caption{CNS}
    \end{subfigure}

    \caption{Log RMSE of AL strategies, measured across 10 rounds of acquisition. Each round incurs constant cost of data acquisition, namely the budget $B$.}
    \label{fig:main}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/burgers.png} % Scaled image
%         \caption{Burgers}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/kdv.png} % Scaled image
%         \caption{KdV}
%     \end{subfigure}
%     % \vspace{0.1cm} % Adjust space between subfigures
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/ks.png} % Scaled image
%         \caption{KS}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}{0.24\textwidth} % Reduced width
%         \centering
%         \includegraphics[width=0.9\textwidth]{figure/main/ns.png} % Scaled image
%         \caption{NS}
%     \end{subfigure}

%     \caption{Log RMSE of AL strategies, measured across 10 rounds of acquisition. Each round incurs constant cost of data acquisition, namely the budget $B$.}
%     \label{fig:main}
% \end{figure*}

==> figure/main_oneline/main_oneline.tex <==

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/main_oneline/heat.png}
        \caption{Heat}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/main_oneline/kdv.png}
        \caption{KdV}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.217\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/main_oneline/ks.png}
        \caption{KS}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/main_oneline/ns.png}
        \caption{NS}
    \end{subfigure}

    \caption{RMSE of AL strategies, measured across 10 rounds of acquisition}
    \label{fig:main_oneline}
\end{figure}


==> figure/pca/pca.tex <==

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/pca/heat.png}
        \caption{Heat}
    \end{subfigure}

    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/pca/kdv.png}
        \caption{KdV}
    \end{subfigure}

    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/pca/ks.png}
        \caption{KS}
    \end{subfigure}
    
    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/pca/ns.png}
        \caption{NS}
    \end{subfigure}

    \caption{PCA of PDE states. Black points are states fully sampled from 10 trajectories. Red points are states randomly sampled from all the states.}
    \label{fig:pca}
\end{figure}


==> figure/stap_pca/stap_pca_ks.tex <==

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/stap_pca/burgers.png}
        \caption{Burgers}
    \end{subfigure}
    % \hfill
    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/stap_pca/kdv.png}
        \caption{KdV}
    \end{subfigure}

    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/stap_pca/ks.png}
        \caption{KS}
    \end{subfigure}
    % \hfill
    % \vspace{0.5cm} % Adjust space between subfigures

    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/stap_pca/ins.png}
        \caption{INS}
    \end{subfigure}
      % \vspace{0.5cm} % Adjust space between subfigures

    \caption{PCA of FNO activation for PDE states sampled by SBAL and SBAL+STAP during the first round of active learning}
    \label{fig:stap_pca}
\end{figure}


==> figure/surrogates/surrogates.tex <==

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/surrogates/qoi.png}
        \caption{QoI prediction}
    \end{subfigure}
    \hspace{0.2cm}
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/surrogates/single.png}
        \caption{Single state prediction}
    \end{subfigure}
    \hspace{0.2cm} % Adjust space between subfigures
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/surrogates/traj.png}
        \caption{Autoregressive trajectory prediction}
    \end{subfigure}
    % \hspace{0.5cm}
    % \begin{subfigure}{0.4\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figure/surrogates/auto.png}
    %     \caption{Autoregressive trajectory prediction}
    % \end{subfigure}

    \caption{Task settings assumed by previous works in active learning of PDEs.}
    \label{fig:surrogates}
\end{figure}


==> figure/timesteps/timesteps.tex <==
% \usepackage{graphicx}
% \usepackage{subcaption}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/timesteps/burgers.png}
        \caption{Burgers}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/timesteps/kdv.png}
        \caption{KdV}
    \end{subfigure}

    \vspace{0.1cm}
    
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/timesteps/ks.png}
        \caption{KS}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/timesteps/ns.png}
        \caption{NS}
    \end{subfigure}
    
    \caption{Timesteps chosen by SBAL+\gls{stap} in the first rounds of active learning, shown for each PDE. Each row corresponds to an acquired trajectory, where yellow cells indicate the selected time steps.}
    \label{fig:timesteps}
\end{figure}


==> table/efficient.tex <==
\begin{table}[t]
\caption{Comparison with more efficient versions of FlexAL. \label{tab:efficient}}
\centering
\begin{tabular}{lcccc}
\toprule
Metric & SBAL & +FlexAL & +FlexAL MF & +FlexAL 10 \\
\midrule
\multicolumn{5}{c}{\textbf{Heat}} \\
\midrule
RMSE & $-5.901 \spm 0.017$ & $\mathbf{-6.304} \spm 0.015$ & $-6.303 \spm 0.009$ & $-6.058 \spm 0.020$ \\
NRMSE & $-6.644 \spm 0.015$ & $\mathbf{-7.014} \spm 0.015$ & $-7.013 \spm 0.010$ & $-6.792 \spm 0.019$ \\
MAE & $-7.699 \spm 0.018$ & $\mathbf{-8.114} \spm 0.015$ & $-8.113 \spm 0.008$ & $-7.858 \spm 0.019$ \\
\midrule
\multicolumn{5}{c}{\textbf{KdV}} \\
\midrule
RMSE & $0.030 \spm 0.029$ & $\mathbf{-0.088} \spm 0.040$ & $-0.065 \spm 0.034$ & $-0.118 \spm 0.024$ \\
NRMSE & $-1.282 \spm 0.030$ & $\mathbf{-1.378} \spm 0.040$ & $-1.350 \spm 0.034 $ & $-1.419 \spm 0.022$ \\
MAE & $-2.139 \spm 0.027$ & $\mathbf{-2.239} \spm 0.043$ & $-2.213 \spm 0.034$ & $-2.273 \spm 0.029$ \\
\midrule
\multicolumn{5}{c}{\textbf{KS}} \\
\midrule
RMSE & $-0.275 \spm 0.014$ & $\mathbf{-0.349} \spm 0.003$ & $-0.326 \spm 0.004$ & $-0.316 \spm 0.009$ \\
NRMSE & $-1.700 \spm 0.014$ & $\mathbf{-1.774} \spm 0.003$ & $-1.752 \spm 0.004$ & $-1.741 \spm 0.009$ \\
MAE & $-2.184 \spm 0.014$ & $\mathbf{-2.265} \spm 0.003$ & $-2.240 \spm 0.005$ & $-2.229 \spm 0.010$ \\
\midrule
\multicolumn{5}{c}{\textbf{NS}} \\
\midrule
RMSE & $-2.052 \spm 0.009$ & $-2.092 \spm 0.003$ & $\mathbf{-2.093} \spm 0.004$ & $-2.078 \spm 0.010$ \\
NRMSE & $-4.253 \spm 0.009$ & $\mathbf{-4.293} \spm 0.003$ & $\mathbf{-4.293} \spm 0.004 $ & $-4.278 \spm 0.011$ \\
MAE & $-4.592 \spm 0.008$ & $-4.632 \spm 0.003$ & $\mathbf{-4.633} \spm 0.004$ & $-4.617 \spm 0.010$ \\
\bottomrule
\end{tabular}

\end{table}


% \begin{table}[htbp]
% \centering
% \begin{tabular}{lcccc}
% \hline
% \rule{0pt}{2ex} Metric & SBAL & +\gls{stap} & +\gls{stap} MF & +\gls{stap} 10 \\
% \hline
% \multicolumn{5}{c}{\textbf{Heat}} \\
% \hline
% RMSE & $-5.901 \spm 0.017$ & $\mathbf{-6.304} \spm 0.015$ & $-6.303 \spm 0.009$ & $-6.058 \spm 0.020$ \\
% NRMSE & $-6.644 \spm 0.015$ & $\mathbf{-7.014} \spm 0.015$ & $-7.013 \spm 0.010$ & $-6.792 \spm 0.019$ \\
% MAE & $-7.699 \spm 0.018$ & $\mathbf{-8.114} \spm 0.015$ & $-8.113 \spm 0.008$ & $-7.858 \spm 0.019$ \\
% \hline
% \multicolumn{5}{c}{\textbf{KdV}} \\
% \hline
% RMSE & $0.030 \spm 0.029$ & $\mathbf{-0.088} \spm 0.040$ & $-0.065 \spm 0.034$ & $-0.118 \spm 0.024$ \\
% NRMSE & $-1.282 \spm 0.030$ & $\mathbf{-1.378} \spm 0.040$ & $-1.350 \spm 0.034 $ & $-1.419 \spm 0.022$ \\
% MAE & $-2.139 \spm 0.027$ & $\mathbf{-2.239} \spm 0.043$ & $-2.213 \spm 0.034$ & $-2.273 \spm 0.029$ \\
% \hline
% \multicolumn{5}{c}{\textbf{KS}} \\
% \hline
% RMSE & $-0.275 \spm 0.014$ & $\mathbf{-0.349} \spm 0.003$ & $-0.326\spm 0.004$ & $-0.316 \spm 0.009$ \\
% NRMSE & $-1.700 \spm 0.014$ & $\mathbf{-1.774} \spm 0.003$ & $-1.752\spm 0.004$ & $-1.741 \spm 0.009$ \\
% MAE & $-2.184 \spm 0.014$ & $\mathbf{-2.265} \spm 0.003$ & $-2.240 \spm 0.005$ & $-2.229 \spm 0.010$ \\
% \hline
% \multicolumn{5}{c}{\textbf{NS}} \\
% \hline
% RMSE & $-2.052 \spm 0.009$ & $-2.092 \spm 0.003$ & $\mathbf{-2.093} \spm 0.004$ & $-2.078 \spm 0.010$ \\
% NRMSE & $-4.253 \spm 0.009$ & $\mathbf{-4.293} \spm 0.003$ & $\mathbf{-4.293} \spm 0.004 $ & $-4.278 \spm 0.011$ \\
% MAE & $-4.592 \spm 0.008$ & $-4.632 \spm 0.003$ & $\mathbf{-4.633} \spm 0.004$ & $-4.617 \spm 0.010$ \\
% \hline
% \end{tabular}
% \caption{Comparison with more efficient versions of \gls{stap} \label{tab:efficient}}
% \end{table}

==> table/main_base.tex <==
\begin{table}[t]
\caption{Results with other base methods}
\label{tab:main_base}
\centering
\begin{tabular}{lcccc}
\toprule
 & Random+\gls{stap} & QbC+\gls{stap} & LCMD+\gls{stap} \\
\midrule
\multicolumn{4}{c}{\textbf{Heat}} \\
\midrule
RMSE & $-6.193 \spm 0.021$ & $-6.195 \spm 0.015$ & $-6.132 \spm 0.024$ \\
NRMSE & $-6.953 \spm 0.017$ & $-6.880 \spm 0.018$ & $-6.843 \spm 0.023$ \\
MAE & $-7.997 \spm 0.021$ & $-8.008 \spm 0.015$ & $-7.944 \spm 0.024$ \\
\midrule
\multicolumn{4}{c}{\textbf{KdV}} \\
\midrule
RMSE & $0.017 \spm 0.042$ & $-0.088 \spm 0.040$ & $-0.103 \spm 0.034$ \\
NRMSE & $-1.292 \spm 0.042$ & $-1.378 \spm 0.040$ & $-1.397 \spm 0.033$ \\
MAE & $-2.162 \spm 0.041$ & $-2.239 \spm 0.043$ & $-2.200 \spm 0.036$ \\
\midrule
\multicolumn{4}{c}{\textbf{KS}} \\
\midrule
RMSE & $-0.259 \spm 0.012$ & $-0.349 \spm 0.003$ & $-0.283 \spm 0.015$ \\
NRMSE & $-1.684 \spm 0.012$ & $-1.774 \spm 0.003$ & $-1.712 \spm 0.013$ \\
MAE & $-2.167 \spm 0.012$ & $-2.265 \spm 0.003$ & $-2.207 \spm 0.013$ \\
\midrule
\multicolumn{4}{c}{\textbf{NS}} \\
\midrule
RMSE & $-2.067 \spm 0.012$ & $-2.092 \spm 0.003$ & $-2.258 \spm 1.119$ \\
NRMSE & $-4.267 \spm 0.012$ & $-4.293 \spm 0.003$ & $-4.218 \spm 0.017$ \\
MAE & $-4.606 \spm 0.012$ & $-4.632 \spm 0.003$ & $-4.559 \spm 0.016$ \\
\bottomrule
\end{tabular}

\end{table}




% \begin{table}[htbp]
% \centering
% \begin{tabular}{lcccc}
% \hline
% \rule{0pt}{2ex} & Random+\gls{stap} & QbC+\gls{stap} & LCMD+\gls{stap} \\
% \hline
% \multicolumn{4}{c}{\textbf{Heat}} \\
% \hline
% RMSE & $-6.193 \spm 0.021$ & $-6.195 \spm 0.015$ & $-6.132 \spm 0.024$ \\
% NRMSE & $-6.953 \spm 0.017$ & $-6.880 \spm 0.018$ & $-6.843 \spm 0.023$ \\
% MAE & $-7.997 \spm 0.021$ & $-8.008 \spm 0.015$ & $-7.944 \spm 0.024$ \\
% \hline
% \multicolumn{4}{c}{\textbf{KdV}} \\
% \hline
% RMSE & $0.017 \spm 0.042$ & $-0.088 \spm 0.040$ & $-0.103 \spm 0.034$ \\
% NRMSE & $-1.292 \spm 0.042$ & $-1.378 \spm 0.040$ & $-1.397 \spm 0.033$ \\
% MAE & $-2.162 \spm 0.041$ & $-2.239 \spm 0.043$ & $-2.200 \spm 0.036$ \\
% \hline
% \multicolumn{4}{c}{\textbf{KS}} \\
% \hline
% RMSE & $-0.259 \spm 0.012$ & $-0.349 \spm 0.003$ & $-0.283 \spm 0.015$ \\
% NRMSE & $-1.684 \spm 0.012$ & $-1.774 \spm 0.003$ & $-1.712 \spm 0.013$ \\
% MAE & $-2.167 \spm 0.012$ & $-2.265 \spm 0.003$ & $-2.207 \spm 0.013$ \\
% \hline
% \multicolumn{4}{c}{\textbf{NS}} \\
% \hline
% RMSE & $-2.067 \spm 0.012$ & $-2.092 \spm 0.003$ & $-2.258 \spm 1.119$ \\
% NRMSE & $-4.267 \spm 0.012$ & $-4.293 \spm 0.003$ & $-4.218 \spm 0.017$ \\
% MAE & $-4.606 \spm 0.012$ & $-4.632 \spm 0.003$ & $-4.559 \spm 0.016$ \\
% \hline
% \end{tabular}
% \caption{Results with other base methods}
% \label{tab:main_base}
% \end{table}


==> table/main_base_partial.tex <==
% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{lcccccc}
% \toprule
%  & \multicolumn{2}{c}{Random} &   \multicolumn{2}{c}{QbC}  &  \multicolumn{2}{c}{LCMD} \\
%  & +\gls{stap} & $\Delta$ & +\gls{stap} &$\Delta$& +\gls{stap} &$\Delta$ \\
% \midrule
% \textbf{Heat}  & $-6.193 \spm 0.021$ & $-0.505 \spm 0.030$ & $-6.195 \spm 0.015$ & $-0.271 \spm 0.029$ & $-6.131 \spm 0.024$ & $-0.390 \spm 0.034$ \\
% % \midrule
% \textbf{KdV}  & $-0.067 \spm 0.054$  & $-0.258 \spm 0.079$ & $0.134 \spm 0.035$ & $-0.132 \spm 0.044$ & $0.286 \spm 0.034$ & $0.030 \spm 0.045$ \\
% % \midrule
% \textbf{KS}  & $-0.335 \spm 0.012$ & $-0.077 \spm 0.012$ & $-0.331 \spm 0.013$ & $-0.063 \spm 0.013$ & $-0.138 \spm 0.016$ & $-0.184 \spm 0.021$ \\
% % \midrule
% \textbf{NS}  & $-2.080 \spm 0.003$ & $-0.030 \spm 0.011$ & $-2.079 \spm 0.008$ & $-0.022 \spm 0.012$ & $-2.05 \spm 0.007$ & $-0.032 \spm 0.018$ \\
% \bottomrule
% \end{tabular}
% \caption{Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement ($\Delta$) over base methods}
% \label{tab:main_base_partial}
% \end{table}


% \begin{table}[t]
% \caption{Transposed Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement over base methods. $\Delta$ refers to the improvements from baselines. Negative $\Delta$ indicates better performance of \gls{stap}.}
% \label{tab:main_base_partial_transposed}
% \setlength{\tabcolsep}{3pt} % Adjust column padding
% \renewcommand{\arraystretch}{0.9} % Adjust row height
% \centering
% \resizebox{0.9\linewidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
%  & \textbf{Heat}          & \textbf{KdV}           & \textbf{KS}            & \textbf{NS}            \\
% \midrule
% \textbf{Random + \gls{stap}} & $-6.193\PM{0.021}$ & $-0.067\PM{0.054}$ & $-0.335\PM{0.012}$ & $-2.080\PM{0.003}$ \\
% \textbf{Random $\Delta$}     & $-0.505\PM{0.030}$ & $-0.258\PM{0.079}$ & $-0.077\PM{0.012}$ & $-0.030\PM{0.011}$ \\
% \textbf{QbC + \gls{stap}}    & $-6.195\PM{0.015}$ & $ 0.134\PM{0.035}$ & $-0.331\PM{0.013}$ & $-2.079\PM{0.008}$ \\
% \textbf{QbC $\Delta$}        & $-0.271\PM{0.029}$ & $-0.132\PM{0.044}$ & $-0.063\PM{0.013}$ & $-0.022\PM{0.012}$ \\
% \textbf{LCMD + \gls{stap}}   & $-6.131\PM{0.024}$ & $ 0.286\PM{0.034}$ & $-0.138\PM{0.016}$ & $-2.050\PM{0.007}$ \\
% \textbf{LCMD $\Delta$}       & $-0.390\PM{0.034}$ & $ 0.030\PM{0.045}$ & $-0.184\PM{0.021}$ & $-0.032\PM{0.018}$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
% \begin{table}[t]
% \caption{Transposed Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement over base methods. $\Delta$ refers to the improvements from baselines. Negative $\Delta$ indicates better performance of \gls{stap}.}
% \label{tab:main_base_partial_transposed}
% \setlength{\tabcolsep}{3pt} % Adjust column padding
% \renewcommand{\arraystretch}{0.9} % Adjust row height
% \centering
% \resizebox{0.9\linewidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Method} & \textbf{Heat}          & \textbf{KdV}           & \textbf{KS}            & \textbf{NS}            \\
% \midrule
% \textbf{Random} \\
% \hspace{1em}\textbf{+ \gls{stap}} & -6.193\PM{0.021} & -0.067\PM{0.054} & -0.335\PM{0.012} & -2.080\PM{0.003} \\
% \multicolumn{1}{c}{\hspace{1em}\textbf{$\Delta$}} & \multicolumn{1}{c}{-0.505\PM{0.030}} & \multicolumn{1}{c}{-0.258\PM{0.079}} & \multicolumn{1}{c}{-0.077\PM{0.012}} & \multicolumn{1}{c}{-0.030\PM{0.011}} \\
% \cmidrule(lr){1-5}
% \textbf{QbC} \\
% \hspace{1em}\textbf{+ \gls{stap}} & -6.195\PM{0.015} & $ 0.134\PM{0.035}$ & -0.331\PM{0.013} & -2.079\PM{0.008} \\
% \multicolumn{1}{c}{\hspace{1em}\textbf{$\Delta$}} & \multicolumn{1}{c}{-0.271\PM{0.029}} & \multicolumn{1}{c}{-0.132\PM{0.044}} & \multicolumn{1}{c}{-0.063\PM{0.013}} & \multicolumn{1}{c}{-0.022\PM{0.012}} \\
% \cmidrule(lr){1-5}
% \textbf{LCMD} \\
% \hspace{1em}\textbf{+ \gls{stap}} & -6.131\PM{0.024} & $ 0.286\PM{0.034}$ & -0.138\PM{0.016} & -2.050\PM{0.007} \\
% \multicolumn{1}{c}{\hspace{1em}\textbf{$\Delta$}} & \multicolumn{1}{c}{-0.390\PM{0.034}} & \multicolumn{1}{c}{$ 0.030\PM{0.045}$} & \multicolumn{1}{c}{-0.184\PM{0.021}} & \multicolumn{1}{c}{-0.032\PM{0.018}} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


\begin{table}[t]
\caption{Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement over base methods. $\Delta$ refers to the improvements from baselines. Negative $\Delta$ indicates better performance of \gls{stap}.}
\label{tab:main_base_partial}
\setlength{\tabcolsep}{3pt} % Adjust column padding
\renewcommand{\arraystretch}{0.9} % Adjust row height
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{llcccc}
\toprule
 &  & \textbf{Burgers}          & \textbf{KdV}           & \textbf{KS}            & \textbf{NS}            \\
\midrule
\multirow{2}{*}{{Random}} & {+ \gls{stap}} & -3.477\PM{0.064} & -0.067\PM{0.054} & -0.335\PM{0.012} & -0.489\PM{0.012} \\
                                   & {$\Delta$}      & -0.596\PM{0.088} & -0.258\PM{0.079} & -0.077\PM{0.012} & -0.067\PM{0.016} \\
\cmidrule(lr){1-6}
\multirow{2}{*}{{QbC}}    & {+ \gls{stap}} & -3.333\PM{0.064} &  \phantom{-}0.134\PM{0.035} & -0.331\PM{0.013} & -0.466\PM{0.011}\\
                                   & {$\Delta$}      & -0.211\PM{0.091} & -0.132\PM{0.044} & -0.063\PM{0.013} & -0.081\PM{0.018} \\
\cmidrule(lr){1-6}
\multirow{2}{*}{{LCMD}}   & {+ \gls{stap}} & -2.925\PM{0.061} &  \phantom{-}0.286\PM{0.034} & -0.138\PM{0.016} & -0.378\PM{0.012}\\
                                   & {$\Delta$}      & -0.078\PM{0.066} &  \phantom{-}0.030\PM{0.045} & -0.184\PM{0.021} & -0.059\PM{0.016} \\
\bottomrule
\end{tabular}%
}
\end{table}



% \begin{table}[t]
% \caption{Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement over base methods. $\Delta$ refers to the improvements from baselines. Negative $\Delta$ indicates better performance of \gls{stap}.
% \label{tab:main_base_partial}}
% % \small
% \setlength{\tabcolsep}{3pt} % Adjust column padding
% \renewcommand{\arraystretch}{0.9} % Adjust row height
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrr}
% \toprule
%  & \multicolumn{2}{c}{Random} &   \multicolumn{2}{c}{QbC}  &  \multicolumn{2}{c}{LCMD} \\
%  \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%  & \multicolumn{1}{c}{+\gls{stap}} & \multicolumn{1}{c}{$\Delta$} & \multicolumn{1}{c}{+\gls{stap}} &\multicolumn{1}{c}{$\Delta$}& \multicolumn{1}{c}{+\gls{stap}} &\multicolumn{1}{c}{$\Delta$} \\
% \midrule
% \textbf{Heat}  & $-6.193 \pm 0.021$ & $-0.505 \pm 0.030$ & $-6.195 \pm 0.015$ & $-0.271 \pm 0.029$ & $-6.131 \pm 0.024$ & $-0.390 \pm 0.034$ \\
% \textbf{KdV}   & $-0.067 \pm 0.054$  & $-0.258 \pm 0.079$ & $0.134 \pm 0.035$ & $-0.132 \pm 0.044$ & $0.286 \pm 0.034$ & $0.030 \pm 0.045$ \\
% \textbf{KS}    & $-0.335 \pm 0.012$ & $-0.077 \pm 0.012$ & $-0.331 \pm 0.013$ & $-0.063 \pm 0.013$ & $-0.138 \pm 0.016$ & $-0.184 \pm 0.021$ \\
% \textbf{NS}    & $-2.080 \pm 0.003$ & $-0.030 \pm 0.011$ & $-2.079 \pm 0.008$ & $-0.022 \pm 0.012$ & $-2.050 \pm 0.007$ & $-0.032 \pm 0.018$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[t]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
%  & Random+\gls{stap} & $\Delta$ &  QbC+\gls{stap} & $\Delta$  & LCMD+\gls{stap} & $\Delta$ \\
% \midrule
% \textbf{Heat}  & $-6.193 \spm 0.021$ & &$-6.195 \spm 0.015$ & &$-6.131 \spm 0.024$& \\
% % \midrule
% \textbf{KdV}  & $-0.067 \spm 0.054$  & &$0.134 \spm 0.035$ & &$0.286 \spm 0.034$ &\\
% % \midrule
% \textbf{KS}  & $-0.335 \spm 0.012$ & &$-0.331 \spm 0.013$ & &$-0.138 \spm 0.016$ &\\
% % \midrule
% \textbf{NS}  & $-2.080 \spm 0.003$ & &$-2.079 \spm 0.008$ & &$-2.05 \spm 0.007$ &\\
% \bottomrule
% \end{tabular}
% \caption{Log RMSE of \gls{stap} averaged across 10 rounds, and their improvement over base methods}
% \label{tab:main_base_partial}
% \end{table}


==> table/quantiles.tex <==
\begin{table}[t]
\caption{RMSE quantiles.}
\label{tab:quantiles}
\centering
\begin{tabular}{lccccc}
\toprule
& Random & QbC & LCMD & SBAL & SBAL+FlexAL \\
\midrule
\multicolumn{6}{c}{\textbf{Heat}} \\
\midrule
99\% & $-4.211 \spm 0.029$ & $-4.848 \spm 0.027$ & $-4.466 \spm 0.027$ & $-4.624 \spm 0.049$ & $\mathbf{-5.284} \spm 0.020$ \\
95\% & $-4.712 \spm 0.022$ & $-5.222 \spm 0.024$ & $-4.945 \spm 0.026$ & $-5.073 \spm 0.035$ & $\mathbf{-5.653} \spm 0.012$ \\
50\% & $-5.992 \spm 0.020$ & $-6.068 \spm 0.024$ & $-5.940 \spm 0.023$ & $-6.111 \spm 0.008$ & $\mathbf{-6.433} \spm 0.014$ \\
\midrule
\multicolumn{6}{c}{\textbf{KdV}} \\
\midrule
99\% & $2.449 \spm 0.011$ & $1.868 \spm 0.006$ & $1.859 \spm 0.007$ & $1.875 \spm 0.017$ & $\mathbf{1.731} \spm 0.022$ \\
95\% & $0.936 \spm 0.012$ & $0.862 \spm 0.018$ & $0.813 \spm 0.011$ & $1.317 \spm 0.014$ & $\mathbf{0.720} \spm 0.018$ \\
50\% & $0.526 \spm 0.014$ & $0.584 \spm 0.011$ & $0.596 \spm 0.012$ & $0.670 \spm 0.008$ & $\mathbf{0.497} \spm 0.019$ \\
\midrule
\multicolumn{6}{c}{\textbf{KS}} \\
\midrule
99\% & $1.097 \spm 0.002$ & $1.042 \spm 0.011$ & $1.077 \spm 0.007$ & $1.086 \spm 0.017$ & $\mathbf{1.060} \spm 0.012$ \\
95\% & $0.478 \spm 0.016$ & $0.404 \spm 0.012$ & $0.439 \spm 0.011$ & $0.463 \spm 0.008$ & $\mathbf{0.431} \spm 0.011$ \\
50\% & $0.068 \spm 0.022$ & $0.041 \spm 0.011$ & $0.082 \spm 0.015$ & $0.098 \spm 0.012$ & $\mathbf{0.083} \spm 0.015$ \\
\midrule
\multicolumn{6}{c}{\textbf{NS}} \\
\midrule
99\% & $-0.959 \spm 0.029$ & $-0.962 \spm 0.006$ & $-0.967 \spm 0.017$ & $-0.988 \spm 0.005$ & $\mathbf{-0.982} \spm 0.008$ \\
95\% & $-1.266 \spm 0.011$ & $-1.261 \spm 0.019$ & $-1.248 \spm 0.022$ & $-1.309 \spm 0.004$ & $\mathbf{-1.303} \spm 0.005$ \\
50\% & $-2.208 \spm 0.016$ & $-2.217 \spm 0.011$ & $-2.168 \spm 0.019$ & $-2.249 \spm 0.011$ & $\mathbf{-2.235} \spm 0.007$ \\
\bottomrule
\end{tabular}

\end{table}


% \begin{table}[htbp]
% \centering
% \begin{tabular}{lccccc}
% \hline
% \rule{0pt}{2ex} & Random & QbC & LCMD & SBAL & SBAL+FlexAL \\
% \hline
% \multicolumn{6}{c}{\textbf{Heat}} \\
% \hline
% 99\% & $-4.211 \spm 0.029$ & $-4.848 \spm 0.027$ & $-4.466 \spm 0.027$ & $-4.624 \spm 0.049$ & $\mathbf{-5.284} \spm 0.020$ \\
% 95\% & $-4.712 \spm 0.022$ & $-5.222 \spm 0.024$ & $-4.945 \spm 0.026$ & $-5.073 \spm 0.035$ & $\mathbf{-5.653} \spm 0.012$ \\
% 50\% & $-5.992 \spm 0.020$ & $-6.068 \spm 0.024$ & $-5.940 \spm 0.023$ & $-6.111 \spm 0.008$ & $\mathbf{-6.433} \spm 0.014$ \\
% \hline
% \multicolumn{6}{c}{\textbf{KdV}} \\
% \hline
% 99\% & $2.449 \spm 0.011$ & $1.868 \spm 0.006$ & $1.859 \spm 0.007$ & $1.875 \spm 0.017$ & $\mathbf{1.731} \spm 0.022$ \\
% 95\% & $0.936 \spm 0.012$ & $0.862 \spm 0.018$ & $0.813 \spm 0.011$ & $1.317 \spm 0.014$ & $\mathbf{0.720} \spm 0.018$ \\
% 50\% & $0.526 \spm 0.014$ & $0.584 \spm 0.011$ & $0.596 \spm 0.012$ & $0.670 \spm 0.008$ & $\mathbf{0.497} \spm 0.019$ \\
% \hline
% \multicolumn{6}{c}{\textbf{KS}} \\
% \hline
% 99\% & $1.097 \spm 0.002$ & $1.042 \spm 0.011$ & $1.077 \spm 0.007$ & $1.086 \spm 0.017$ & $\mathbf{1.060} \spm 0.012$ \\
% 95\% & $0.478 \spm 0.016$ & $0.404 \spm 0.012$ & $0.439 \spm 0.011$ & $0.463 \spm 0.008$ & $\mathbf{0.431} \spm 0.011$ \\
% 50\% & $0.068 \spm 0.022$ & $0.041 \spm 0.011$ & $0.082 \spm 0.015$ & $0.098 \spm 0.012$ & $\mathbf{0.083} \spm 0.015$ \\
% \hline
% \multicolumn{6}{c}{\textbf{NS}} \\
% \hline
% 99\% & $-0.959 \spm 0.029$ & $-0.962 \spm 0.006$ & $-0.967 \spm 0.017$ & $-0.988 \spm 0.005$ & $\mathbf{-0.982} \spm 0.008$ \\
% 95\% & $-1.266 \spm 0.011$ & $-1.261 \spm 0.019$ & $-1.248 \spm 0.022$ & $-1.309 \spm 0.004$ & $\mathbf{-1.303} \spm 0.005$ \\
% 50\% & $-2.208 \spm 0.016$ & $-2.217 \spm 0.011$ & $-2.168 \spm 0.019$ & $-2.249 \spm 0.011$ & $\mathbf{-2.235} \spm 0.007$ \\
% \hline
% \end{tabular}
% \caption{RMSE quantiles}
% \label{tab:quantiles}
% \end{table}


==> table/regularization.tex <==

\begin{table}[t]
\caption{Effect of regularization \label{tab:regularization}}
\centering
\begin{tabular}{lcccc}
\toprule
 & SBAL & +\gls{stap} & +Pushforward & +Gaussian \\
\midrule
\multicolumn{5}{c}{\textbf{Burgers}} \\
\midrule
RMSE & $-3.388 \spm 0.052$ & $\mathbf{-3.674} \spm 0.071$ & $-0.879 \spm 0.020$ & $-3.371 \spm 0.053$ \\
NRMSE & $-4.081 \spm 0.061$ & $\mathbf{-4.306} \spm 0.065$ & $-1.419 \spm 0.032$ & $-4.069 \spm 0.056$ \\
MAE & $-5.332 \spm 0.046$ & $\mathbf{-5.585} \spm 0.066$ & $-2.712 \spm 0.024$ & $-5.313 \spm 0.052$ \\
\midrule
\multicolumn{5}{c}{\textbf{KdV}} \\
\midrule
RMSE & $0.030 \spm 0.029$ & $\mathbf{-0.088} \spm 0.040$ & $0.924 \spm 0.613$ & $0.017 \spm 0.042$ \\
NRMSE & $-1.282 \spm 0.030$ & $\mathbf{-1.378} \spm 0.040$ & $-0.245 \spm 0.689$ & $-1.292 \spm 0.042$ \\
MAE & $-2.139 \spm 0.027$ & $\mathbf{-2.239} \spm 0.043$ & $-1.077 \spm 0.690$ & $-2.162 \spm 0.041$ \\
\midrule
\multicolumn{5}{c}{\textbf{KS}} \\
\midrule
RMSE & $-0.275 \spm 0.014$ & $\mathbf{-0.349} \spm 0.003$ & $1.148 \spm 0.795$ & $-0.259 \spm 0.012$ \\
NRMSE & $-1.700 \spm 0.014$ & $\mathbf{-1.774} \spm 0.003$ & $-0.283 \spm 0.792$ & $-1.684 \spm 0.012$ \\
MAE & $-2.184 \spm 0.014$ & $\mathbf{-2.265} \spm 0.003$ & $-0.473 \spm 0.956$ & $-2.167 \spm 0.012$ \\
\midrule
\multicolumn{5}{c}{\textbf{INS}} \\
\midrule
RMSE & $-0.461 \spm 0.012$ & $\mathbf{-0.525} \spm 0.005$ & $1.374 \spm 0.047$ & $-0.462 \spm 0.010$ \\
NRMSE & $-2.751 \spm 0.012$ & $\mathbf{-2.814} \spm 0.005$ & $-0.915 \spm 0.047$ & $-2.751 \spm 0.009$ \\
MAE & $-2.736 \spm 0.009$ & $\mathbf{-2.797} \spm 0.003$ & $-0.884 \spm 0.039$ & $-2.737 \spm 0.007$ \\
\midrule
\multicolumn{5}{c}{\textbf{CNS}} \\
\midrule
RMSE & $2.422 \spm 0.045$ & $\mathbf{2.363} \spm 0.016$ & $4.446 \spm 0.014$ & $2.44 \spm 0.046$ \\
NRMSE & $-2.482 \spm 0.040$ & $\mathbf{-2.501} \spm 0.051$ & $-0.318 \spm 0.026$ & $-2.476 \spm 0.049$ \\
MAE & $-0.880 \spm 0.041$ & $\mathbf{-0.932} \spm 0.015$ & $0.997 \spm 0.013$ & $-0.864 \spm 0.045$ \\
\bottomrule
\end{tabular}

\end{table}



% \begin{table}[htbp]
% \centering
% \begin{tabular}{lcccc}
% \hline
% \rule{0pt}{2ex}  & SBAL & +\gls{stap} & +Pushforward & +Gaussian \\
% \hline
% \multicolumn{5}{c}{\textbf{Heat}} \\
% \hline
% RMSE & $-5.901 \spm 0.017$ & $\mathbf{-6.304} \spm 0.015$ & $-3.086 \spm 1.584$ & $-5.844 \spm 0.011$ \\
% NRMSE & $-6.644 \spm 0.015$ & $\mathbf{-7.014} \spm 0.015$ & $-3.755 \spm 1.627$ & $-6.558 \spm 0.013$ \\
% MAE & $-7.699 \spm 0.018$ & $\mathbf{-8.114} \spm 0.015$ & $-4.884 \spm 1.583$ & $-7.630 \spm 0.012$ \\
% \hline
% \multicolumn{5}{c}{\textbf{KdV}} \\
% \hline
% RMSE & $0.030 \spm 0.029$ & $\mathbf{-0.088} \spm 0.040$ & $0.924 \spm 0.613$ & $0.017 \spm 0.042$ \\
% NRMSE & $-1.282 \spm 0.030$ & $\mathbf{-1.378} \spm 0.040$ & $-0.245 \spm 0.689$ & $-1.292 \spm 0.042$ \\
% MAE & $-2.139 \spm 0.027$ & $\mathbf{-2.239} \spm 0.043$ & $-1.077 \spm 0.690$ & $-2.162 \spm 0.041$ \\
% \hline
% \multicolumn{5}{c}{\textbf{KS}} \\
% \hline
% RMSE & $-0.275 \spm 0.014$ & $\mathbf{-0.349} \spm 0.003$ & $1.148 \spm 0.795$ & $-0.259 \spm 0.012$ \\
% NRMSE & $-1.700 \spm 0.014$ & $\mathbf{-1.774} \spm 0.003$ & $-0.283 \spm 0.792$ & $-1.684 \spm 0.012$ \\
% MAE & $-2.184 \spm 0.014$ & $\mathbf{-2.265} \spm 0.003$ & $-0.473 \spm 0.956$ & $-2.167 \spm 0.012$ \\
% \hline
% \multicolumn{5}{c}{\textbf{NS}} \\
% \hline
% RMSE & $-2.052 \spm 0.009$ & $\mathbf{-2.092} \spm 0.003$ & $-0.060 \spm 1.118$ & $-2.067 \spm 0.012$ \\
% NRMSE & $-4.253 \spm 0.009$ & $\mathbf{-4.293} \spm 0.003$ & $-2.258 \spm 1.119$ & $-4.267 \spm 0.012$ \\
% MAE & $-4.592 \spm 0.008$ & $\mathbf{-4.632} \spm 0.003$ & $-2.619 \spm 1.107$ & $-4.606 \spm 0.012$ \\
% \hline
% \end{tabular}
% \caption{Effect of Regularization \label{tab:regularization}}
% \end{table}
